Parton Distributions

We provide an assessment of the state of the art in various issues related to experimental measurements, phenomenological methods and theoretical results relevant for the determination of parton distribution functions (PDFs) and their uncertainties, with the specific aim of providing benchmarks of different existing approaches and results in view of their application to physics at the LHC. We discuss higher order corrections, we review and compare different approaches to small x resummation, and we assess the possible relevance of parton saturation in the determination of PDFS at HERA and its possible study in LHC processes. We provide various benchmarks of PDF fits, with the specific aim of studying issues of error propagation, non-gaussian uncertainties, choice of functional forms of PDFs, and combination of data from different experiments and different processes. We study the impact of combined HERA (ZEUS-H1) structure function data, their impact on PDF uncertainties, and their implications for the computation of standard candle processes, and we review the recent F_L determination at HERA. Finally, we compare and assess methods for luminosity measurements at the LHC and the impact of PDFs on them.

==> tab_hl.tex <==
\begin{table}[ht]
  \begin{center}
    \begin{tabular}{|l|r|}
      \hline
      Name & $\chi^2/N_{\rm data}$ \\
      \hline
      ZEUS97  &  1.09 \\
      H1lowx97  &  1.03 \\
      NMC     &  1.40 \\
      NMC\_pd &  1.24 \\
      BCDMS   &  1.21 \\
      \hline
      Total &  1.19 \\
      \hline
    \end{tabular}
  \end{center}
\caption{NNPDF $\chi^2$ for the total and each single data set.\label{tab:nnpdf_chi2_bench1}
}
\end{table}

